Adapt in Contexts: Retrieval-Augmented Domain Adaptation via In-Context Learning

Large language models (LLMs) have showcased their capability with few-shot inference known as in-context learning. However, in-domain demonstrations are not always readily available in real scenarios, leading to cross-domain in-context learning. Besides, LLMs are still facing challenges in long-tail knowledge in unseen and unfamiliar domains. The above limitations demonstrate the necessity of Unsupervised Domain Adaptation (UDA). In this paper, we study the UDA problem under an in-context learning setting to adapt language models from the source domain to the target domain without any target labels. The core idea is to retrieve a subset of cross-domain elements that are the most similar to the query, and elicit language model to adapt in an in-context manner by learning both target domain distribution and the discriminative task signal simultaneously with the augmented cross-domain in-context examples. We devise different prompting and training strategies, accounting for different LM architectures to learn the target distribution via language modeling. With extensive experiments on Sentiment Analysis (SA) and Named Entity Recognition (NER) tasks, we thoroughly study the effectiveness of ICL for domain transfer and demonstrate significant improvements over baseline models.

==> llama_ner_rand_demo.tex <==
\begingroup
\begin{table*}[hb]
    \centering
    \caption{
    Example input and output pairs for Alpaca-Lora on NER dataset BC2GM. Demonstrations are randomly sampled from CoNLL03.
    }
    \vspace{2.8mm}
    \begin{tabular}{p{0.96\linewidth}}
        \toprule
Please identify all entities from the input sentence. If there is no entity, please output None.\\
\vspace{-2mm}
Sentence: The 32-year-old defender played seven seasons with Nantes and was with Paris St Germain for five seasons . \\
Entity: Nantes, Paris St Germain \\
Sentence: 29,582 \\
Entity: None \\
Sentence: The Palestinian Authority was set up under the 1993 PLO-Israel interim peace deal .\\
Entity: Palestinian Authority, PLO-Israel\\
Sentence: In Home Health said it previously recorded a reserve equal to 16 percent of all revenue related to the community liaison costs . \\
Entity: In Home Health \\
Sentence: " I realised this year , that without putting 99.9 percent of your mind into tennis , I do n't think you can successful , " said the 22-year-old Medvedev .\\
Entity: Medvedev \\
\vspace{-2mm}
\textbf{Sentence:} Physical mapping 220 kb centromeric of the human MHC and DNA sequence analysis of the 43 - kb segment including the RING1 , HKE6 , and HKE4 genes .\\
\textbf{Entity:} \\
human MHC, RING1, HKE6, HKE4.\\
\vspace{2mm}


Please identify all entities from the input sentence. If there is no entity, please output None.\\
\vspace{-2mm}
Sentence: The blue-chip CAC-40 index ended 2.43 points or 0.12 percent lower at 2,017.99 points after a brief foray into positive territory when the New York stock market opened higher . \\
Entity: CAC-40, New York \\
Sentence: American League \\
Entity: American League \\
Sentence: 1886 - At Skeleton Canyon in Arizona , Geronimo , Apache chief and leader of the last great Red Indian rebellion finally surrendered to General Nelson Miles . \\
Entity: Skeleton Canyon, Arizona, Geronimo, Red Indian, Nelson Miles \\
Sentence: ( Formula Shell leads best-of-seven series 1-0 ) \\
Entity: Formula Shell\\
Sentence: PRESS DIGEST - Jordan - Aug 25 .
Entity: Jordan
\vspace{-2mm}
\textbf{Sentence:} DNA elements recognizing NF - Y and Sp1 regulate the human multidrug - resistance gene promoter .\\
\textbf{Entity:} \\
NF-Y, Sp1, DNA elements. \\

\bottomrule
    \end{tabular}
\end{table*}
\endgroup
